DarkGates: A Hybrid Power-Gating Architecture to Mitigate the Performance Impact of Dark-Silicon in High Performance Processors

To reduce the leakage power of inactive (dark) silicon components, modern processor systems shut-off these components' power supply using low-leakage transistors, called power-gates. Unfortunately, power-gates increase the system's power-delivery impedance and voltage guardband, limiting the system's maximum attainable voltage (i.e., Vmax) and, thus, the CPU core's maximum attainable frequency (i.e., Fmax). As a result, systems that are performance constrained by the CPU frequency (i.e., Fmax-constrained), such as high-end desktops, suffer significant performance loss due to power-gates. To mitigate this performance loss, we propose DarkGates, a hybrid system architecture that increases the performance of Fmax-constrained systems while fulfilling their power efficiency requirements. DarkGates is based on three key techniques: i) bypassing on-chip power-gates using package-level resources (called bypass mode), ii) extending power management firmware to support operation either in bypass mode or normal mode, and iii) introducing deeper idle power states. We implement DarkGates on an Intel Skylake microprocessor for client devices and evaluate it using a wide variety of workloads. On a real 4-core Skylake system with integrated graphics, DarkGates improves the average performance of SPEC CPU2006 workloads across all thermal design power (TDP) levels (35W-91W) between 4.2% and 5.3%. DarkGates maintains the performance of 3DMark workloads for desktop systems with TDP greater than 45W while for a 35W-TDP (the lowest TDP) desktop it experiences only a 2% degradation. In addition, DarkGates fulfills the requirements of the ENERGY STAR and the Intel Ready Mode energy efficiency benchmarks of desktop systems.

==> 8_discussion.tex <==
\section{Discussion}\label{sec:discussion}

In this paper we present a hybrid power-gating architecture to mitigate the voltage drop due to the increased system impedance that exists in motherboard voltage regulators (MBVR \cite{rotem2011power,10_jahagirdar2012power,11_fayneh20164,12_howse2015tick}) power delivery networks. MBVR PDN is used in several recent client processors, such as Skylake \cite{anati2016inside,haj2016fine}, Kaby Lake \cite{kabylake_2020},  Coffee Lake \cite{coffeelake_2020}, and Cannon Lake \cite{i38121u_cannonlake}. 
Other recent high-end client processor use integrated voltage regulators (IVR \cite{2_burton2014fivr,5_nalamalpu2015broadwell,tam2018skylake,icelake2020}), and low dropout voltage regulators (LDO \cite{singh20173,singh2018zen,burd2019zeppelin,beck2018zeppelin,toprak20145,sinkar2013low} ). The power switches inside the IVR and LDO voltage regulators are used as power-gates to shut-off the power supplies of the target components (e.g., a CPU core) \cite{2_burton2014fivr,beck2018zeppelin}. While IVR and LDO PDNs mitigate part of the system impedance issue by regulating the voltage near the load (e.g., CPU cores) and by sharing board and package resources \cite{haj2020flexwatts,haj2019comprehensive}, there PDNs introduce new design tradeoff that adds voltage guardband and multiple challenges and  to the system \cite{naffziger2016integrated,yen2016all}. 

First, due to the reduced available decoupling capacitance (decap) on die and package per voltage domain (e.g., CPU core), IVR and LDO VRs implement  faster transient load response, which typically requires high clock frequency (e.g., $>100MHz$ \cite{yang20150}). The high frequency results in high power losses which decreases the power-conversion efficiency. As such, and \emph{voltage guardband} is added to compensate on voltage fluctuations due to load transient \cite{haj2020flexwatts}.   


Second, IVR design scalability is challenging due to the difficulty to scale the traditional analog designs \cite{2_burton2014fivr,beck2018zeppelin,haj2020flexwatts} 
designs. LDO is less energy efficient than MBVR architecture in workloads that have high voltage difference between the power domains, such as between CPU cores and graphics engines in computer graphics workloads \cite{haj2020flexwatts,haj2019comprehensive}.

Third, IVR and LDO can increase  the die temperature due to the power conversion losses on these on-chip regulator \cite{naffziger2016integrated,haj2020flexwatts}. The increased temperature  reduced the effective system TDP, which can increase the leakage power consumption and reduce the performance of thermally constrained system \cite{naffziger2016integrated}.   




==> README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> backups/2_background_backup.tex <==
\section{Background}\label{sec:background}

We provide a brief background on the architecture, power delivery networks, and design limits in modern client processors such as \om{Intel} Skylake \cite{anati2016inside,haj2016fine}, Kaby Lake \cite{kabylake_2020}, Coffee Lake \cite{coffeelake_2020}, and Cannon Lake \cite{i38121u_cannonlake}. 


%\subsection{Modern Processor Architecture}
% \noindent \textbf{Scope.} 
% %{Techniques for current management}  {exist} in most modern processors of different segments (e.g., smartphones, client, servers), {built by different} vendors (e.g., Intel, ARM, AMD). {They also exist in} processors with different power delivery networks {, such as} motherboard voltage regulators (MBVR \cite{rotem2011power,10_jahagirdar2012power,11_fayneh20164,12_howse2015tick}), integrated voltage regulators (IVR \cite{singh20173,singh2018zen,burd2019zeppelin,beck2018zeppelin,toprak20145,sinkar2013low}), and low dropout voltage regulators (LDO \cite{2_burton2014fivr,5_nalamalpu2015broadwell,tam2018skylake,icelake2020}){.}
% {I}n this work{,} we \emph{{only}} focus on recent client processor of Intel that uses  motherboard voltage regulators power delivery network for CPU cores (e.g., Skylake \cite{anati2016inside}, Kabylake \cite{kabylake_2020}, CoffeeLake \cite{coffeelake_2020}, CannonLake \cite{i38121u_cannonlake}). 
% %r{Why? Are there similarities with other processors/vendors...?}

%architecture to explain the  architectures The processor architecture that we use is similar to Intel client processor architecture~\cite{2_burton2014fivr, rotem2012power, anati2016inside, burres2015intel, meinerzhagen2018energy }.

\subsection{Client Processor Architecture}\label{sec:client_arch}
A high-end client processor is a system-on-chip (SoC) that typically integrates three main domains 
into a single chip: 1) compute (e.g., CPU
cores and graphics engines), 2) IO, and 3) memory {system}. 
Fig. \ref{microarch}(a) shows the architecture used in recent Intel processors (e.g., Skylake \cite{11_fayneh20164},   Coffee Lake \cite{coffeelake_2020}, and Cannon Lake \cite{i38121u_cannonlake}{)}  with a focus on CPU cores. 
% The Fig. show{s} three main components of a processor with two CPU cores: 1) power delivery, 2) clocking, and 3) power management. 


\begin{figure}[ht]
\begin{center}
\includegraphics[trim=0.5cm 0.6cm 0.5cm 0.6cm, clip=true,width=0.9\linewidth,keepaspectratio]{figs/arch.pdf}
\caption{(a) Architecture overview of recent Intel client processors. All cores share the same voltage regulator (VR). Each {CPU} core has a {power-gate} (PG) for the entire core. (b) Package layout showing an ungated main voltage domain ($V_{CU}$) arriving from the CPU \om{core} VR that feeds four power-gated voltage domains (one for each CPU core, $V_{C0G}$, $V_{C1G}$, $V_{C2G}$, $V_{C3G}$). (c) Side view of die and package showing 1) the ungated main voltage domain ($V_{CU}$) and two cores\om{'} voltage domains ($V_{C0G}$ and  $V_{C1G}$), and 2) the package's decoupling capacitors \cite{15_jakushokas2010power}.}\label{microarch}
\end{center}
%  \vspace{-15pt}
\end{figure}




\noindent \textbf{Power Management.} The processor includes one central power management unit (PMU) and one local PMU per CPU core. The central PMU is responsible for several power-management activities, such as dynamic voltage and frequency scaling~{\cite{gonzalez1996energy,haj2018power,hajsysscale,rotem2011power}}. 
The central PMU has several interfaces \om{to} on-chip and off-chip components{,} such as to
1) the motherboard VR, i.e., serial voltage identification (\emph{SVID}) \cite{rotem2012power,rotem2015intel,haj2018power,gough2015cpu}, to control the voltage level of the VR, 
2) the phase-locked-loop\js{,} to control the clock frequency,
and 3) each core's local PMU\om{, to} communicat\om{e} power management commands and status \om{report}. 
The local PMU inside the CPU core is responsible for core-specific power management, such as clock gating, power gating control, thermal reporting.

\noindent \textbf{Clocking.} A phase-locked loop (PLL) suppl{ies} the clock {signal to {all} CPU {cores.}  {All}}  CPU cores {have} the same {maximum} clock frequency \cite{8th_9th_gen_intel,icelake2020,perf_limit_reasons,haj2018energy}.\footnote{Typically, Intel client processors \om{that} use {fully-integrated voltage regulator (FIVR)} power delivery, \om{including Haswell and {Ice Lake} {processors},} have the same clock frequency domain for all cores \cite{6_kanter2013haswell,icelake2020}.} 

\noindent \textbf{Power Gating.}
Power gating is a circuit-level technique to significantly reduce \om{the} leakage power of an idle circuit \cite{hu2004microarchitectural,haj2018power,gough2015cpu}. 
A power-gate is implemented using low-leakage transistors that \om{shut off} the input voltage to the target circuit and comes with a \emph{power-area tradeoff}. A power-gate needs to be large enough to help reduce i) the power delivery impedance ($R$), ii) the voltage drop (i.e., $IR$ drop), and iii) the operating voltage and power consumption of the target circuit when it is active. However, a power-gate for a large circuit (\om{e.g.,} a CPU core) can \om{consume significant} chip area \cite{zelikson2011embedded,shockley1952unipolar,petrica2013flicker,ditomaso2017machine,rahman2006determination,flynn2007low}.
A power-gate may involve an additional trade-off between leakage power consumption reduction and performance loss due to the latency to ungate the circuit (i.e., open the power gate). 
Typically, the wake-up latency from the {power-gated} state can take a handful to tens of cycles \cite{kahng2013many,gough2015cpu}. However, to reduce the worst-case peak in-rush current \cite{chadha2013architectural,usami2009design,agarwal2006power,abba2014improved} and voltage noise of power-delivery (e.g., di/dt noise {\cite{larsson1997di,gough2015cpu,haj2018power}}) when waking up a power-gate, {the {power-gate} controller applies} a \emph{staggered} wake-up {technique} \cite{agarwal2006power} that takes tens of nanoseconds (typically, $10$--$20ns$) \cite{kahng2013many,akl2009effective,kahng2012tap}.

\begin{sloppypar}
\noindent \textbf{Power Budget Management (PBM).}
To keep the system running below a TDP limit, the \om{SoC PMU} employs a \emph{power budget management \js{(PBM)}} algorithm to dynamically distribute the total power budget to each SoC domain \cite{lempel20112nd,rotem2013power,rotem2012power,21_doweck2017inside,ranganathan2006ensemble,rotem2011power,zhang2016maximizing,isci2006analysis,hajsysscale,ananthakrishnan2014dynamically,haj2020flexwatts}. This allows each domain to operate within its allocated power budget.
For instance, CPU cores and graphics engines in the compute domain share the same power budget. When a graphics-intensive workload is executed, the graphics engines consume most of the compute domain's power budget. \end{sloppypar}

To keep the power consumption of the compute domain within its allocated power budget, PMU applies  dynamic voltage and frequency scaling (DVFS) to 1) reduce the CPU cores' power consumption and 2) increase {the} graphics engines' {performance}   \cite{rotem2013power,rotem2012power,kim2008system,rotem2015intel}.


\begin{sloppypar}
\noindent \textbf{System Idle Power States (C-states).}
%\head{SoC Power States (C-states)}
The Advanced Configuration and Power Interface (ACPI\footnote{\om{ACPI} is an industry standard that is widely used for OS-directed configuration, power management, and thermal management of computing {systems}.}) defines a processor's \emph{idle power states}, commonly called \emph{C-states}~\cite{acpi}.
C-states are defined in two {primary} levels:
1) the component level, such as thread ($TCi$), core ($CCi$), and graphics ($RCi$) C-states, and 2) the system level, known as \emph{package C-states} ($PCi$ or $Ci$)~\cite{intel_skl_dev,haj2018power}.
\end{sloppypar}


A package C-state defines an idle power state of the system (consisting of the processor, chipset, external memory devices). A system enters a specific package C-state depending on each system component's idle power state (\emph{component C-state}). 
Various levels of package C-states exist to provide a range of power consumption levels with various techniques, such as clock gating at the uncore level, or a nearly {complete} shutdown of the system. 
The ACPI standard includes recommendations on the C-states, but manufacturers are free to define their C-states and the \om{corresponding} system behavior at each C-state.
In this work, we focus on the package C-states of the Intel Skylake architecture \cite{intel_skl_dev}, but similar idle power state definitions exist in other architectures (e.g.,  AMD{\cite{amd_specs}} and ARM {\cite{qcom2018}}). 
Table~{\ref{tab:p-states}} shows all package C-states of the Intel Skylake architecture and the major conditions under which the power management unit (PMU) places the system into each package C-state (a similar table exists in the Intel manual{\cite{intel_skl_dev}}). 
%Table~{\ref{tab:p-states}} also shows the entry/exit latencies for each package C-state, which are measured on a real system.

Typical \emph{desktop} systems based on processors prior to Skylake, support up to \emph{package $C7$} (e.g., Haswell \cite{bolla2016assessing,hammarlund2014haswell}, Broadwell \cite{mosalikanti2015low}), while mobile systems  support up to $C10$ (e.g., Haswell-ULT \cite{kurd2014haswell}, Broadwell-ULX \cite{deval2015power}).   

\input{pc_table}

%\head{Power Levels of Package C-states} 
% The system's  power level (in Watts) in each package C-state depends on the operating points (e.g., voltage and frequency) of the active components in the power state. 
% For example, the power level at $C0$ state depends on how many cores or graphics engines are active and their operating voltages/frequencies. 
% Similarly, the power level at $C8$ state depends on the display resolution that the DC and {eDP} are driving (the higher the resolution, the higher the DC clock frequency and voltage).

\subsection{Client Processor Packages and Die Sharing}

Architects of modern  client processors typically build a \emph{single} CPU core (with a built-in power-gate) architecture\footnote{An Intel CPU core has nearly the same {microarchitecture} for client and server processors. Intel CPU core design is a single development project, leading to a master superset core. Each project has two derivatives, one for server and one for client processors~\cite{Skylake_die_server}.} that supports \emph{all} \om{dies} of a client processor family, and some of the \om{dies} are used to build different processor packages targeting different segments. For example, the Intel Skylake processor for high-end \emph{mobile} (i.e., Skylake-H \cite{Skylake_H}) processors and high-end \emph{desktop} (i.e., Skylake-S \cite{Skylake_D}) uses a single processor die   \cite{skl_dies,tam2018skylake,21_doweck2017inside} for all TDP ranges (from  $35W$ \cite{intel_skl__3_5} to $91W$ \cite{intel_skl_91}). Recent AMD  client processors use \om{a} similar strategy \cite{singh20173,singh2018zen,burd2019zeppelin,beck2018zeppelin,amd_zen2_10,amd_zen2_54}.
This design reuse is adopted for two major reasons.  
First,  doing so allows system manufacturers to configure a processor for a specific segment using two main methods: 1) By configuring processor's TDP (known as configurable TDP \cite{cTDP,cTDP2,jahagirdar2012power} or cTDP) to enable the  processor to operate at higher or lower performance levels, depending on the available cooling capacity and desired power consumption of the system. 2) By integrating one or more dies (e.g., \om{CPU} dies, chipset, embedded-DRAM) into a single package that is optimized for a specific market segment. For example, a land grid array (LGA \cite{kujala2002transition}) package for desktops and a ball grid array (BGA \cite{guenin1995analysis}) package for laptops.     
Second, it reduces non-recurring engineering (NRE \cite{magarshack2003system}) cost and design complexity to  allow competitive product prices and enable the meeting of strict time-to-market requirements. 




\subsection{Power Delivery {Network} (PDN)} 
There are three commonly-used PDNs in recent high-end client processors~\om{\cite{haj2020flexwatts}}: motherboard voltage regulators (MBVR \cite{rotem2011power,10_jahagirdar2012power,11_fayneh20164,12_howse2015tick}), integrated voltage regulators (IVR \cite{singh20173,singh2018zen,burd2019zeppelin,beck2018zeppelin,toprak20145,sinkar2013low}), and low dropout voltage regulators (LDO \cite{2_burton2014fivr,5_nalamalpu2015broadwell,tam2018skylake,icelake2020}). 
We describe aspects of the MBVR PDN here due to its simplicity. 
%Sec. \ref{sec:discussion} discusses the IVR and LDO PDNs.
As shown in Fig. \ref{microarch}(a), the MBVR PDN of a high-end client processor includes 1) one motherboard voltage regulator (VR) for all CPU cores, 2) {a} \emph{load-line} impedance ($R_{LL}${)}, and  3) power-gates for each individual core.\footnote{Fine-grain\om{ed} power-gates exist in a CPU core\om{. F}or example\om{,} a power-gate is implemented \om{in} each AVX unit (e.g., AVX512~{\cite{mandelblat2015technology,intel_avx512}}) inside a CPU core.} All CPU cores share the same VR \cite{rotem2011power,10_jahagirdar2012power,11_fayneh20164,12_howse2015tick,haj2018energy}{.} For more details on state-of-the-art PDNs, we refer the reader to our \om{recent} prior work~\cite{haj2020flexwatts}.


% en  clocking (Phase-locked loop, or PLL)  and central/local power management units (PMU).  The central PMU communicates with the Cores VR using a dedicated interface called serial voltage ID (SVID) \cite{rotem2012power}. All cores share the same VR (i.e., Core VR) \cite{rotem2011power,10_jahagirdar2012power,11_fayneh20164,12_howse2015tick}) and each core have a power gate (PG) to turn-off the entire core when it's idle \cite{rotem2012power}. While  each AVX unit inside the core (e.g., AVX512 \cite{intel_avx512}) has a PG \cite{mandelblat2015technology}. All  CPU cores share the same clock frequency\footnote{All Intel client processors, including Haswell and the new Icelake processors which uses FIVR power delivery, have the same clock frequency domain for all cores \cite{6_kanter2013haswell,icelake2020}. } \cite{8th_9th_gen_intel,icelake2020,perf_limit_reasons}.





% There are three commonly-used PDNs in recent high-end client processors: motherboard voltage regulators (MBVR \cite{9_rotem2011power,10_jahagirdar2012power,11_fayneh20164,12_howse2015tick}), integrated voltage regulators (IVR \cite{singh20173,singh2018zen,burd2019zeppelin,beck2018zeppelin,toprak20145,sinkar2013low}), and low dropout voltage regulators (LDO \cite{2_burton2014fivr,5_nalamalpu2015broadwell,tam2018skylake,icelake2020}).



%\subsection{Loadline, Voltage Guardband, and Voltage Limits}\label{loadline_gb}

% \noindent \textbf{Dynamic and Static Current.} 
% Equation \ref{eqn:current} shows the current consumption, denoted by $Icc$,  of CMOS design \cite{haj2018power,gough2015cpu}. $Icc$ consists of two major components, leakage current ($Icc_{lkg}$) and dynamic current ($Icc_{dyn}$). $Icc_{lkg}$ is proportional to 1) the supply voltage ($Vcc$), 2) number of  design's transistors (e.g., number of powered-on cores) power by the supply voltage, and 3) temperature. $Icc_{dyn}$ is proportional to 1) the dynamic capacitance ($C_{dyn}$, where $C_{dyn}= \alpha \cdot C$ ){,} which is affected mainly by the the amount of design capacitance ($C$) and the node transition activity factor\footnote{A node transition activity factor, is a statistical parameter and is data rate dependent{. It} defines the probability of the gate's output to make logic transition during one clock cycle.}, denoted by $\alpha$, 2) supply voltage ($Vcc$), and 3) the frequency of the design ($F$).        

% \begin{equation}\label{eqn:current}
% \resizebox{.7\hsize}{!}{$
% Icc = Icc_{lkg} + Icc_{dyn} =  Icc_{lkg} + C_{dyn} \cdot Vcc \cdot F
% $}\end{equation}




\noindent \textbf{Load-line.} {Load-line} or \emph{{adaptive voltage positioning}} \cite{14_module2009and,intel_avp_2009,sun2006novel,tsai2015switching} is a model that describes the voltage and current relationship\footnote{In this model, short current bursts {result} in voltage droops~{\cite{cho2016postsilicon,reddi2009voltage,reddi2010voltage}}{,} which are filtered out by the decoupling capacitors~\cite{peterchev2006load}, while long current bursts are detected by the motherboard VR.} under a given system impedance, denoted by $R_{LL}$. {Fig. \ref{loadline}(a) describes a simplified power delivery network (PDN) model with a voltage regulator (VR), load-line ($R_{LL}$), and load (CPU Cores).} 
{$R_{LL}$ is} typically {$1.6m$--$2.4m\Omega$} for recent client processors \cite{8th_9th_gen_intel,haj2020flexwatts}. The voltage at the load is defined as: $Vcc_{load} =  Vcc - R_{LL}\cdot Icc$, where $Vcc$ and $Icc$ are the voltage and current at the VR output, respectively{, as shown in Fig. \ref{loadline}(b)}. 
From this equation, we can {observe} that the voltage at the load input ($Vcc_{load}$) decreases when the load's current ($Icc$) increases.
Due to this phenomenon, the PMU increases the input voltage ($Vcc$), i.e., {applies} a \emph{voltage guardband}, to a level that keeps the voltage at the load ($Vcc_{load}$) above the minimum functional voltage (i.e., $Vcc_{min}$) under even the most intensive load (i.e., when all {active} cores {are running} a workload that exercises the highest possible dynamic capacitance ($C_{dyn}$){{)}. This workload is} known as a \emph{power-virus} \cite{haj2015compiler,fetzer2015managing,haj2020flexwatts} {and} results in the maximum possible current ($Icc_{virus}$). A typical application consumes a lower current $Icc_{typical}$ than $Icc_{virus}$. The minimal current that the processor can consume is the leakage current ($Icc_{lkg}$) once the clocks are gated (while the supply {voltage} is \emph{not} {power-gated}). In all cases where the current is lower than $Icc_{virus}$, the voltage drop (i.e., $Icc \cdot R_{LL}$) is smaller than when running a power-virus, which results in a higher load voltage $Vcc_{load}$ than necessary (as shown in {Fig. \ref{loadline}(b)}){, leading to a power loss that increases quadratically with the voltage level.} 


\begin{figure}[ht]
\begin{center}
\includegraphics[trim=0.8cm 0.99cm 0.8cm 0.8cm, clip=true,width=1\linewidth,keepaspectratio]{figs/loadline.pdf}\\
\caption{Adaptive voltage guardband on modern processors. (a) Simplified Power Delivery Network (PDN) model with a load-line. {(b) Voltage at the load is defined as: $Vcc_{load} =  Vcc - R_{LL}\cdot Icc$, where $Vcc$ and $Icc$ are the voltage and current at the VR output, respectively.} {(c)} Multi-level load-line with three power{-}virus levels. The voltage guardband is adjusted based on the power{-}virus level corresponding to {the} \om{system} state of the processor (e.g., number of active cores {and instructions' computational intensity}).}\label{loadline}
\end{center}
% \vspace{-15pt}
\end{figure}

\begin{sloppypar}
\noindent \textbf{Adaptive Voltage Guardband, Icc$_{max}$, and Vcc$_{max}$.} To reduce the power loss {resulting} from a high voltage guardband when \emph{not} running a power-virus, due to the load-line effect, modern processors define \emph{multiple levels} of power-viruses depending on the maximum dynamic capacitance ($C_{dyn}$) that a \om{system} state (e.g., number {of} active cores, the computational intensity of running instructions) can draw. 
For each power{-}virus level, the processor applies {a} \emph{different} voltage guardband.  
%Power delivery network (PDN) of a processor handles short current conjunctions by the filter capacitor network on die, package and board \cite{zu2015adaptive}. For a high current event to be observed by the board and VR, it needs to last hundreds of nanoseconds to a few microseconds (few hundreds to a few thousands of core clock cycles), depending on PDN design. With this observation, the VR and its connection to the processor is shown in the simplified model of Fig. 3. 
%Fig. \ref{loadline}(a) describes a simplified power delivery network (PDN) model with load-line. The load-line or Adaptive Voltage Positioning (AVP) \cite{intel_avp_2009,sun2006novel,tsai2015switching} describes the behavior of the load voltage ($Vcc_{load}$) as it appears to the VR and motherboard\footnote{In this model, short current bursts results in voltage droops which are filtered out by the decoupling capacitors, while long current burst are observed by the motherboard VR}. $Vcc_{load}$ is the supply 
Fig. \ref{loadline}{(c)} illustrates the load-line model behavior of a processor with three power-virus levels denoted by $VirusLevel_1$, $VirusLevel_2$, and  $VirusLevel_3$ (where $VirusLevel_1 < VirusLevel_2 < VirusLevel_3$). The three power-virus levels represent multiple scenarios. For example, $VirusLevel_1$, $VirusLevel_2$,  and $VirusLevel_3$ can represent one, two, or four active cores, respectively, for a processor with four cores. 
When the processor moves from one power-virus level to a higher/lower level, the processor increases/decreases the voltage by a voltage guardband ($\Delta V$). For example, when moving from $VirusLevel_1$ to  $VirusLevel_2$, the processor increases the voltage by $\Delta V_2$ as shown ({in} blue {text}) in Fig. \ref{loadline}{(c)}.
\end{sloppypar}


\subsection{Processor Design Limits}

\subsubsection{Thermal Limits}
\om{W}e \om{describe} the most important thermal limits that constrain the performance on modern processors. 

\noindent \textbf{Junction Temperature ($T_{jmax}$) Limit.}
As the processor dissipates power, the temperature of the silicon junction ($T_j$) increases\om{.} 
\js{$T_j$} should be kept below the maximum junction temperature ($T_{jmax}$) \om{as o}verheating may cause permanent damage to the processor. \om{T}he  processor measures the temperature and applies multiple \om{techniques (e.g., PBM~\cite{lempel20112nd}, thermal throttling~\cite{haj2018power}, and catastrophic trip temperature~\cite{gough2015cpu})} to ensure that the temperature remains under the $T_{jmax}$ limit. In the worst case, the processor automatically shut\om{s} down when the silicon \om{junction} temperature reache\om{s} its operating limit \cite{haj2018power,haj2018energy,rotem2015intel,intel_xtu_overclocking,intel_avp_2009}.


% \noindent \textbf{Skin Temperature Limit.} 
% The device skin (surface) temperature can limit its performance. In small form-factor mobile devices (such as smartphones and tablets) skin temperature can reach high levels that can cause burns on the device user even before the while junction temperature reaches the limit (i.e., $T_{jmax}$). Hence, thermal design and management are crucial for a mobile device to maximize performance and energy efficiency while maintaining safe temperatures \cite{xie2014therminator,rotem2015power}.

\noindent \textbf{Thermal Design Power (TDP).}
TDP (in watts) is the \om{maximum} sustainable power consumption under the maximum theoretical load (e.g., common applications, but not a power-virus) that the cooling solution \om{of the system} needs to be designed for \cite{xie2014therminator,rotem2015power,isci2006analysis,haj2018power,cTDP,cTDP2}.

\subsubsection{Power Delivery Network (PDN) Limits}\label{sec:pdn_limits}
There are multiple PDN limits in \om{a} modern processor\om{.} \om{W}e \om{describe} the most important \om{ones}. 

\noindent \textbf{VR Thermal Design Current (TDC).}
TDC is the the continuous load current, also known as maximum continuous current, thermal current, or second power limit (i.e., PL2 \cite{rotem2015intel}). TDC is the sustained current that the processor is capable of drawing indefinitely and defines the current to use for the voltage regulator (VR) temperature assessment. In other words, TDC is the amount of electrical current the VR must \om{be able to} supply \om{while being} thermally viable \cite{intel_tdc,burd2019zeppelin,su2017high}\om{.} 


\noindent \textbf{Power Supply and Battery Maximum Current Limit.}
The power supply unit (e.g., ATX power supply \cite{meisner2009powernap}, power brick \cite{rotem2015intel}\om{)} and/or device battery that \om{supply} current to the system VRs also \om{have} current limits. For example, the third power limit (i.e., PL3) is used \hj{for battery over-current protection} \cite{rotem2015intel}.  




\noindent \textbf{VR Electrical Design Current (EDC) Limit.}
The  power delivery of a modern processor is limited by EDC, also known as \om{the} maximum instantaneous current, peak current, $Icc_{max}$, or fourth power limit (i.e., PL4 \cite{rotem2015intel}). EDC is \om{the} maximum amount of current at any instantaneous short period of time that can be delivered by a motherboard VR or an integrated VR (e.g., FIVR \cite{2_burton2014fivr}). EDC limit is typically imposed by the limited maximum current that the VRs can supply \cite{gough2015cpu,2_burton2014fivr,haj2018power,skylakex,intel_avp_2009,naffziger2016integrated}.
Exceeding \js{the} EDC limit can result in irreversible damage to the VR, the \om{processor} chip, or tripping VR's protection mechanism for \js{excessive current} that shutdown\om{s} the system. Therefore, a combination of \emph{proactive} enforcement and platform design constraints must be used to prevent system failure~\cite{gough2015cpu,2_burton2014fivr,haj2018power,skylakex,intel_avp_2009,naffziger2016integrated,wright2006characterization,piguet2005low,zhang2014architecture,su2017high}.



\noindent \textbf{Maximum Current per Bump/Pin.} 
The amount of current that a processor's die/package can consume per voltage domain is limited by the maximum current a bump/pin can support \cite{wright2006characterization,piguet2005low,zhang2014architecture}. For example, while integrated VRs mitigate the EDC limit by enabling a reduced input current for the processor \cite{haj2020flexwatts}, the maximum current of \om{the processor} can be limited by the maximum current for a bump/pin.

\noindent \textbf{Minimum Operating Voltage Limit ($V_{min}$).}
Operating below the $V_{min}$ limit can \om{cause} a processor \om{to malfunction}. Therefore, modern processors implement multiple techniques to prevent the voltage from dropping below  $Vcc_{min}$ due to, for example, \emph{di/dt} voltage fluctuations~\om{\cite{joseph2003control,gough2015cpu,haj2018power,reddi2010voltage,reddi2009voltage, brooks2001dynamic,lefurgy2011active}}.



\noindent \textbf{Maximum Operational Voltage Limit ($V_{max}$).}
Technology scaling has made modern integrated circuits more susceptible to \om{reliability} degradation phenomena such as Negative Bias Temperature Instability (NBTI), Electromigration (EM) and Time Dependent Dielectric Breakdown (TDDB) \cite{hu1996gate}. Degradation depends
on many processes and environmental factors, but can be controlled by managing the circuit's temperature and voltage levels \cite{mercati2013workload}. Processor manufacturers define a maximum operational voltage limit ($V_{max}$) that should not be exceeded to ensure the guaranteed processor lifespan and reliability. For example, Intel allows exceeding $V_{max}$ when overclocking a system (e.g., via the BIOS \cite{intel_bios_overclocking} or the XTU tool \cite{intel_xtu_overclocking}). This process is out of the processor's reliability specification and can shorten the processor's lifespan~\cite{intel_bios_overclocking,intel_xtu_overclocking,intel_avp_2009}.

\noindent \textbf{Voltage Droop Effect on Maximum Frequency ($F_{max}$).}
In an active CPU core, simultaneous operations in memory \om{and/or} logic circuits demand high current flow, which creates fast transient voltage droops from the nominal voltage ($V_{nom}$). The worst\om{-}case voltage droop can degrade the maximum attainable frequency at a given voltage since this requires additional voltage (droop) guardband ($V_{gb}$) above the nominal voltage to enable the CPU core to run at the target frequency. In case that the core voltage with the voltage guardband is higher than $V_{max}$ (i.e., $V_{nom} + V_{gb} > V_{max}$) the power management unit reduces $F_{max}$, thereby reducing $V_{nom}$ to keep the CPU core voltage below $V_{max}$. Therefore, voltage guardband ($V_{gb}$) has a direct effect on the CPU core $F_{max}$.       

% \noindent {\textbf{Voltage and Current Limit Protection.}}
% {When dynamically {increasing} the voltage guardband due to moving to a {higher} power-virus level, the processor {may} reduce the cores' frequency 1) {to} keep the voltage within the maximum operational voltage (i.e., $Vcc_{max}$ {in} Fig. \ref{loadline}{(c)}{, pink dashed ellipse)}, and 2) {to} keep the current ($Icc$ in Fig. \ref{loadline}{(b)}) consumed from the VR within the maximum current {limit} ($Icc_{max}$\footnote{{$Icc_{max}$ limit is the maximum current the VR must be electrically designed to support. Exceeding the $Icc_{max}$ limit can result in irreversible damage to the VR or the processor chip \cite{gough2015cpu,intel_opt_ref_manual2020}.}})~\cite{gough2015cpu,2_burton2014fivr,haj2018power,skylakex,intel_avp_2009,naffziger2016integrated,wright2006characterization,piguet2005low,zhang2014architecture}.}

% \noindent \textbf{Voltage Emergency (di/dt) {Avoidance}.}
% {When dynamically moving to a higher power-virus level, the processor increases the cores{'} voltage guardband to {prevent the} voltage {from} dropping below the minimum {operating} voltage (i.e., $Vcc_{min}$ {in} Fig. \ref{loadline}{(c)}{, red dashed {ellipses}}) due to high \emph{di/dt} voltage fluctuations~{\cite{joseph2003control,gough2015cpu,haj2018power,reddi2010voltage,reddi2009voltage}}{.}} 




% the processor  
% {When dynamically adapting (increasing/decreasing) the voltage guardband due to moving to a new virus level, the processor reduce{s} the core's frequency 1) {to} keep}

% Supply voltage fluctuations \cite{joseph2003control,gough2015cpu,haj2018power,haj2015compiler} have emerged as a serious cause for concern in high performance processor design. These perturbations occur when the processor demands rapid changes in load current over a relatively small time scale, known as the \emph{di/dt}. 
% Since the power delivery system has substantial parasitic inductance, this current variation produces voltage ripples on the chip's supply lines. This is significant because if the supply voltage rises/drops above/below a specific tolerance range (i.e., $Vcc_{max}$/$Vcc_{min}$) , the processor may malfunction.




% $Icc_{max}$ limit is the maximum current the VR must be electrically designed to support. Exceeding the the $Icc_{max}$ limit can result in irreversible damage to the VR or the processor's chip. Therefore, a combination of proactive enforcement and platform design constraints must be used to prevent system failure \cite{gough2015cpu,2_burton2014fivr,haj2018power,skylakex,intel_avp_2009,naffziger2016integrated,wright2006characterization,piguet2005low,zhang2014architecture}.
%In modern processors there are much more levels which differentiate between types of instructions set used (e.g., scalar, SSE, AVX2, AVX512) in which each instruction set have different maximum dynamic capacitance.  


% We can observe from Fig. \ref{loadline}(b) 
% %{what is this Fig.? where did you get the results from? explain it first.} 
% that a typical workload, consuming $Icc_{typlical}$ current, runs with a reduced load voltage ($\Delta V_2$ lower voltage)  ($Vcc_{load}$) when running with the $Vcc_1$ voltage, corresponding to $VirusLevel_1$ (green curve) compared when running with a $Vcc_2$ voltage, corresponding to  $VirusLevel_2$ (orange curve).
% When the processor's current exceeds the virus current of $VirusLevel_1$, i.e., $Icc_{virus1}$ (e.g., when additional core is activated) the processor must increase the voltage to a higher level (i.e., $VirusLevel_2$) to keep the load voltage above $Vcc_{min}$ limit. Similarly, when the processor's current exceeds the virus current of $VirusLevel_2$ (i.e., $Icc_{virus2}$){,} the processor must increase the voltage a higher level (i.e., $VirusLevel_3$) to keep the load voltage above $Vcc_{min}$ limit. However, when increasing the voltage guardband to $VirusLevel_3${,} we observe that load voltage can \emph{exceed} the maximum operational voltage (i.e., $Vcc_{max}$) limit, which impacts the reliability of the processor. In this case{,} the processor reduces its current by reducing the operations frequency to keep voltage within safe limits.


% \noindent \textbf{Parameters Affecting {the} Voltage Guardband.}
% {When moving from {the} power-virus level,  $VirusLevel_1$ to a higher level,  $VirusLevel_2$, the voltage guardband {($\Delta V$)}, that should be added to the supply voltage level corresponding to $VirusLevel_1$ {({$Vcc_1$})}, is correlated {with} the difference in current consumption between the two levels, {($Icc_2 - Icc_1$)}. As shown in Equation \ref{eqn:guardband}, $\Delta V $ is proportional to 1) the CPU core frequency, $F$, 2) the {supply voltage level corresponding to $VirusLevel_1$}, {$Vcc_1$}, 3) the load-line impedance, $R_{LL}$, and 4) the difference between core dynamic {capacitances} of the two power-virus {levels}, $C_{dyn2} -  C_{dyn1}$}.    

% \begin{equation}\label{eqn:guardband}
% \resizebox{.7\hsize}{!}{$
% \begin{array}{c}
% \Delta V = Vcc_2 - Vcc_1 \approx (Icc_2 - Icc_1) \cdot R_{LL} \\[\jot]
% = (C_{dyn2} \cdot Vcc_1 \cdot F -  C_{dyn1} \cdot Vcc_1 \cdot F) \cdot R_{LL} \\[\jot]
% = (C_{dyn2} -  C_{dyn1}) \cdot Vcc_1 \cdot F \cdot R_{LL}
% \end{array}
% $}\end{equation}

% The dynamic capacitance of the CPU cores at a given point in time
% %, shown in Equation \ref{eqn:cdyn}, 
% is correlated {with} the 1) number of \emph{active cores}, 2) the \emph{capacitance}, $C$, of each core, and 3) the node \emph{activity factor} of each core. The capacitance, C, of a core is a function of the computational intensity (e.g., MOV, OR, ADD, MULL, FMA) and width (e.g., 64{-}bit scalar, 128{-}bit vector, 256{-}bit vector, 512{-}bit vector) {of the instructions executed by} the cores.   

% \begin{equation}\label{eqn:cdyn}
% \resizebox{.4\hsize}{!}{$
% \begin{array}{c}
% C_{dyn} = \sum_{i=1}^{\#Cores} \alpha \cdot C_i 
% \end{array}
% $}\end{equation}


% active  AVP keeps the load voltage close to the maximum allowed voltage, $V_{max}$ when the load current is low (e.g., when the processor is idle and cosumes only leakage current $I_{Leakage}$. Load voltage will drop to voltage level close to the minimum functional voltage, $V_{min}$, when the load current is at the maximum current that a processor can draw when running a sequence of instruction. 

% Instruction sequence which uses high power demand instructions (e.g., vector instruction) can draw higher maximum current than low power demand instruction (e.g., scalar instruction). To save power in common case, modern processors have different voltage guardband levels corresponding to the instruction category that is being use by the processor at runtime. Fig. \ref{loadline}(b) shows three levels for voltage guardband corresponds to three categories of instruction, for example, \emph{scalar} instructions as first level, \emph{128-bits vector} as second level, and \emph{256-bits vector} instructions as third level.



%AVP allows reducing the power consumption at high loads by reducing the load voltage as shown in Fig. \ref{loadline}. 


%The lowest allowable voltage Vmin is determined by the maximum processor current (Imax) that can be drawn at a given frequency, as this Imax current determines the initial voltage guardband that compensates for voltage droop once this high cur-rent occurs. If we can limit or reduce Imax then we will be able to reduce the voltage guardband to a lower voltage level for the same current. As shown in Fig. 3, the maximum current is Imax\_High. If we can limit the maximum current to Imax\_Low, then workloads with current between Ileakage and Imax\_Low can run with voltage lower by V than the baseline voltage. This will save power consumption in proportion to the square of the load voltage, and in power-constrained modes we will be able to use this “freed” power budget to raise processor frequency and to gain higher perfor-mance relative to the baseline. In this study, we characterize program code regions based on the maximum current that can be drawn. 


%\subsection{Voltage Emergencies (dI/dt)}  \label{sec:didt}
 
%This fundamental challenge is known as the \emph{dI/dt} problem since the magnitude of these voltage ripples are affected by the instantaneous change of current with respect to time.

%\subsection{Power Gating} \label{sec:powergating}

% \subsection{Thermal Design Current (TDC)}
% Thermal {d}esign {c}urrent (TDC) is the the continuous load current, also known as maximum continuous current, or thermal {c}urrent. TDC is the sustained current that the processor is capable of drawing indefinitely and defines the current to use for the voltage regulator temperature assessment. In other words, TDC is the amount of electrical current voltage regulator must supply and be thermally viable . 

%\subsection{Icc$_{max}$ Limit}
% \noindent \textbf{Icc$_{max}$ Limit.}
% The power delivery of a modern processor is limited by {e}lectrical {d}esign {c}urrent (EDC), also known as, maximum instantaneous current, peak current or $Icc_{max}$. $Icc_{max}$ is the the maximum amount of current at any instantaneous short period of time that can be delivered by the motherboard's voltage regulators (VRs). $Icc_{max}$ limit {is} typically {imposed by} 1) the limited maximum current that the VRs can supply \cite{gough2015cpu,2_burton2014fivr,haj2018power,skylakex,intel_avp_2009,naffziger2016integrated}, and 2) the limited current per bump/pin that the die/ package can support \cite{wright2006characterization,piguet2005low,zhang2014architecture}. 
% $Icc_{max}$ limit is the maximum current the VR must be electrically designed to support. Exceeding the the $Icc_{max}$ limit can result in irreversible damage to the VR or the processor's chip. Therefore, a combination of proactive enforcement and platform design constraints must be used to prevent system failure \cite{gough2015cpu,2_burton2014fivr,haj2018power,skylakex,intel_avp_2009,naffziger2016integrated,wright2006characterization,piguet2005low,zhang2014architecture}.


% {The EDC of modern processors can be more than $1.5\times$ the TDC \cite{naffziger2016integrated,21_doweck2017inside}, a}s the processor applies more effective average power reduction mechanisms{, such as} r{are all the next examples of effective average power reduction mechanisms?} power gating of execution units \cite{skylakex,tam2018skylake,21_doweck2017inside}, adding heavy-power instructions (e.g., wide vector instructions), increasing IPC and, running higher frequencies for short term boost (e.g., Turbo Boost techniques {\cite{rotem2012power,21_doweck2017inside,rotem2015intel,amd_zen2_10,singh2018zen,singh20173}}).

% \subsection{Instructions Power}

% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table}[]
% \centering
% \caption{Energy per instruction (EPI) for several Haswell CPU instructions}
% \label{tab:my-table}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lll}
% \hline
% \textbf{\begin{tabular}[c]{@{}l@{}}Instruction \\ Type\end{tabular}} & \textbf{Description} & \textbf{\begin{tabular}[c]{@{}l@{}}Normalized \\ EPI\end{tabular}} \\ \hline
% FMA256   & fused multiply–add 256bit      & 98.2 \\
% Store256 & Vector store of 256bit         & 87.8 \\
% Load256  & Vector load of 256bit          & 70.8 \\
% Store128 & Vector store of 128bit         & 59.1 \\
% Load128  & Vector load of 128bit          & 50.8 \\
% FMA128   & fused multiply–add 128bit      & 48.8 \\
% FMUL128  & Floating-point multiply 128bit & 38.0 \\
% FADD128  & Floating-point Add of 128bit   & 33.9 \\
% IMUL64   & Integer multiply of 64bit      & 10.8 \\
% IMUL32   & Integer multiply of 32bit      & 5.7  \\
% IADD32   & Integer add of 32bit           & 2.1  \\
% MOV32    & Registers Move of 32bit        & 1   
% \end{tabular}%
% }
% \end{table}

